Bayesian History Reconstruction of Complex Human Gene Clusters on a Phylogeny

Clusters of genes that have evolved by repeated segmental duplication present difficult challenges throughout genomic analysis, from sequence assembly to functional analysis. Improved understanding of these clusters is of utmost importance, since they have been shown to be the source of evolutionary innovation, and have been linked to multiple diseases, including HIV and a variety of cancers. Previously, Zhang et al. (2008) developed an algorithm for reconstructing parsimonious evolutionary histories of such gene clusters, using only human genomic sequence data. In this paper, we propose a probabilistic model for the evolution of gene clusters on a phylogeny, and an MCMC algorithm for reconstruction of duplication histories from genomic sequences in multiple species. Several projects are underway to obtain high quality BAC-based assemblies of duplicated clusters in multiple species, and we anticipate that our method will be useful in analyzing these valuable new data sets.

==> Makefile <==
all: figures main.pdf

clean:
	-rm main.aux main.bbl main.blg main.log main.log main.lot main.out \
	main.dvi main.ps main.pdf *~
	make -C figures clean

main.ps: main.dvi
	dvips main -o main.ps

main.pdf: main.dvi
	dvips -Ppdf -G0 main -o main.ps
	ps2pdf main.ps

main.dvi: figures main.tex *.tex *.bib
	latex main
	latex main
	-bibtex main
	latex main
	latex main

.PHONY: figures all

figures:
	#make -C figures

